Non-contact Dexterous Micromanipulation with Multiple Optoelectronic Robots

Micromanipulation systems leverage automation and robotic technologies to improve the precision, repeatability, and efficiency of various tasks at the microscale. However, current approaches are typically limited to specific objects or tasks, which necessitates the use of custom tools and specialized grasping methods. This paper proposes a novel non-contact micromanipulation method based on optoelectronic technologies. The proposed method utilizes repulsive dielectrophoretic forces generated in the optoelectronic field to drive a microrobot, enabling the microrobot to push the target object in a cluttered environment without physical contact. The non-contact feature can minimize the risks of potential damage, contamination, or adhesion while largely improving the flexibility of manipulation. The feature enables the use of a general tool for indirect object manipulation, eliminating the need for specialized tools. A series of simulation studies and real-world experiments -- including non-contact trajectory tracking, obstacle avoidance, and reciprocal avoidance between multiple microrobots -- are conducted to validate the performance of the proposed method. The proposed formulation provides a general and dexterous solution for a range of objects and tasks at the micro scale.

==> chapters/system_design.tex <==
The projection accuracy of the OET is crucial for the successful completion of manipulation tasks. We first establish a OET manipulation platform that realizes closed-loop control with high projection precision and a wide field of view. As depicted in Fig \ref{fig:system}, the platform consists of an optical system, a motion stage, a microfluidic chip, and an AC generator. A schematic of the optical system is shown in Fig. 1(a), which comprises projection, illumination, and observation pathways. The projection pathway is formed by a digital micromirror device (DMD) projector (TI DLP6500) coupled with a projection lens, precisely projecting light patterns computed on the PC side onto the chip. The observation pathway consists of a 20X objective lens (Olympus UPLFLN20X), a tube lens (SWTLU-C), and a 4K CCD camera (LBAS U3120-23C), used to capture microscope images with a wide field of view and transmit them to the PC. The same objective lens serves for both projection and observation, with optimal illumination achieved by fine-tuning the positioning of two convex lenses. The XYZ three-dimensional motor motion stage is used to locate and focus on the target object. We employ an automatic focusing technique based on the energy of the image (ENE) \cite{}, which quantitatively measures image defocus using the ENE sharpness evaluation function and iteratively adjusts the focal length based on the level of defocus until optimal focus is achieved. We manually select the robot and the target object first, and then utilize channel and spatial relatibility tracking (CSRT) \cite{} to stabilize tracking and precisely extract the positions of both amidst changing light and cluttered backgrounds.

\begin{figure}[thb]

    \centering    \includegraphics[width=8.5cm]{fig/system2.png}

    \caption{}

    \label{fig:system}
\end{figure}

The OET chip is illustrated in Fig. 2, which depicts a tri-layer architecture: top, middle, and bottom. The top layer consists of 0.7-$mm$-thick transparent glass coated with a 200-$nm$ layer of indium-tin oxide (ITO). The bottom layer is 1-$mm$-thick ITO glass with a 1-$\mu m$-thick hydrogenated amorphous silicon (a-H:Si) film deposited via plasma-enhanced chemical vapor deposition (PECVD) from Leeliven Instruments Hassrode Shale \cite{Zhang:17}. A microfluidic space with a an approximate height of 100 $\mu m$ is established in the middle layer for operational tasks. The alternating current (AC) power electrodes are respectively connected to the top and bottom layers of the chip, generating an alternating electric field within the microfluidic space. Metallo-dielectric Janus particles (JPs) are employed as robots driven by the OETs. The target objects can consist of consubstantial microparticles or cells. When subjected to the alternating electric field of the OET, the robot and target object pair undergo polarization, resulting in the formation of induced electric dipoles. The light spot projected onto the bottom surface of the OET chip induces a high electric field region. Consequently, the robot experiences non-uniform polarization and is subject to positive bidirectional dielectrophoretic forces (p-DEP). Meanwhile, the homogeneous robot and target object in close proximity experience electrostatic repulsive forces.
